EvoMisty: Building, Optimizing, and Evolving Capabilities on a Social Robot

Social robots face diverse and changing tasks in companionship and education. LLM-based methods can generate task programs, but they still rely on manually developed control interfaces and predefined capabilities. They also lack a general mechanism to optimize completed tasks based on user-specified metrics and reuse performance improvements across tasks.We present EvoMisty, a plugin-based framework that enables coding agents to build and continually improve robot capabilities. EvoMisty builds a control program from official documentation and verifies candidate capabilities on a physical robot. Verified capabilities are stored in an atomic capability library and combined with existing skills to solve tasks. After task completion, EvoMisty can collect execution data, measure user-specified metrics, and iteratively improve task programs. It then distills reusable skills from final solutions into a skill library for future tasks.We evaluate EvoMisty on a physical Misty II robot using Claude Code and Codex. The two agents construct 109 and 107 verified atomic capabilities, respectively. Both complete all 28 AutoMisty benchmark tasks and seven additional tasks beyond AutoMisty's capabilities. Optimization improves all seven evaluated metrics across five tasks. For example, dialogue response latency decreases by 52% and 71%, respectively. Reusing skills from one optimized dialogue task reduces latency by 33% to 72% in three other dialogue tasks without further optimization.

==> sec/supp_A_build.tex <==
\section{Build: Capability Verification on the Robot}
\label{sec:supp-build}

In Sec.~4.1 of the main paper, EvoMisty builds a control program from the official documentation and verifies the candidate capabilities on the physical robot; Table 1 of the main paper reports the results. This section adds two points about how this verification proceeded. \cref{sec:supp-build-repair} reports what happened when capabilities could not be verified with the first version of the control program. \cref{sec:supp-build-examples} shows two verification examples, one that passed and one that failed, and the evidence that decided each.

\subsection{Repairing the Control Program after Failed Verification}
\label{sec:supp-build-repair}

The Build stage in Fig.~2 of the main paper contains a loop: when a verification on the physical robot fails, the agent determines whether the failure is caused by missing functionality in the control program; if so, it adds that functionality and verifies the capability again. This section reports how the loop occurred in our experiments.

Table~1 of the main paper reports 109 and 107 verified capabilities. Of these, 105 (Claude Code) and 103 (Codex) passed with the first version of the control program and never entered the loop. The remaining four passed only after going through it, and they are the same four for both agents: \suppcode{Start\allowbreak Video\allowbreak Streaming}, \suppcode{Stop\allowbreak Video\allowbreak Streaming}, \suppcode{Start\allowbreak Av\allowbreak Streaming}, and \suppcode{Stop\allowbreak Av\allowbreak Streaming}.

The official documentation lists these four interfaces alongside the other HTTP requests and event subscriptions. Following it, the first version of the control program implemented only HTTP requests and event subscriptions; it could not receive video frames and had no RTSP receiver, so the tests for these four capabilities could not be run. EvoMisty recorded them as capabilities that could not be verified because the control program lacked functionality, added video-frame reception and RTSP stream capture to the control program, and verified them again. All four passed.

\subsection{Two Verification Examples: One Passed, One Failed}
\label{sec:supp-build-examples}

\begin{figure}[t]
\begin{suppverifycard}{suppgreen}{suppgreenbg}{\textbf{\textcolor{suppgreen}{Verified}}\hspace{0.55em}\textbf{Video capabilities} (Claude Code and Codex)}
\suppfirstvlabel{Capabilities}
\suppcode{SaveVideo}, \suppcode{GetVideoList}, \suppcode{GetVideo}, \suppcode{DeleteVideo}, \suppcode{DisplayVideo}, \suppcode{SetVideoDisplaySettings}
\suppvlabel{Test input}
A test video that EvoMisty generated itself with \suppcode{ffmpeg}.
\suppvlabel{Evidence}
\textit{File operations.} EvoMisty uploaded, listed, downloaded, and deleted the video; the downloaded file was identical to the uploaded one.

\textit{On-screen effect.} The program cannot observe the screen, so EvoMisty asked the person after playing the video and again after hiding it. The answer was yes both times.
\suppvlabel{Outcome}
All six capabilities verified and added to the Atomic Capability Library.
\end{suppverifycard}
\vspace{5pt}
\begin{suppverifycard}{suppred}{suppredbg}{\textbf{\textcolor{suppred}{Not verified}}\hspace{0.55em}\suppcode{\bfseries DriveTrack} (Codex)}
\suppfirstvlabel{Capability}
\suppcode{DriveTrack}: driving by left and right track speeds.
\suppvlabel{Test}
Three attempts, at track speeds of 10 and then 20.
\suppvlabel{Evidence}
Each command returned success.

The encoder velocities stayed at zero.

The person, when asked, answered that the robot had not moved.
\suppvlabel{Outcome}
Not verified and not added to the Atomic Capability Library.
\end{suppverifycard}
\caption{Two verification examples from Build: one that passed (top) and one that failed (bottom), with the evidence that decided each.}
\label{fig:supp-verify}
\end{figure}

What differs between the two examples in \cref{fig:supp-verify} is the evidence. A successful response does not count as passing by itself: objective evidence or a person's confirmation is also required. This is why Build verifies capabilities on the physical robot: even when every response is normal, the actual state of the robot may not be what the response suggests.


==> sec/supp_B_optimize.tex <==
\begin{table*}[t]
\caption{EvoMisty with Claude Code on Naughty-Child Dialogue: changes kept, in order.}
\label{tab:supp-run}
\supptablesetup
\begin{tabularx}{\textwidth}{|l|>{\raggedright\arraybackslash}X|c|c|}
\hline
\textbf{Stage targeted} & \textbf{Change} & \textbf{Latency (s)} & \textbf{CER} \\
\hline
Speech recognition & Speech recognition now runs locally on the computer. & 6.53\,\supparr\,5.85 & 0.02\,\supparr\,0.00 \\
\hline
Reply generation, speech synthesis & The reply is output while it is being generated; the first sentence is synthesized and played first. & 5.85\,\supparr\,4.70 & 0.00 \\
\hline
Reply generation, upload & A faster dialogue model is used; the audio is compressed before it is uploaded. & 4.70\,\supparr\,4.07 & 0.00 \\
\hline
Speech synthesis & Speech synthesis now runs locally on the computer; the audio is played directly after upload. & 4.07\,\supparr\,3.28 & 0.00 \\
\hline
Retrieving the recording & Speech is now recorded with the computer's microphone, so the recording no longer has to be retrieved from Misty. & 3.28\,\supparr\,2.54 & 0.00 \\
\hline
\end{tabularx}
\supptablenote{Latency and CER are measured inside the Optimize loop. The values in Table~2 of the main paper are measured independently on test data that is never used during optimization.}
\end{table*}

\section{Optimize: From Measurements to an Improved Robot Program}
\label{sec:supp-optimize}

Table~2 of the main paper reports the metrics of five tasks before and after optimization. This section first follows one complete optimization run to illustrate the Optimize loop in Fig.~2 of the main paper (\cref{sec:supp-opt-run}). It then lists, for all five tasks, what the hooks record and which changes were kept in the final programs (\cref{sec:supp-opt-hooks}). Finally, it reports what happens when the same agents optimize the same programs without EvoMisty (\cref{sec:supp-opt-noevo}).

\subsection{One Optimization Run in Detail}
\label{sec:supp-opt-run}

This subsection uses Naughty-Child Dialogue with Claude Code as the example.

\paragraph{How It Is Measured.}
EvoMisty first has a person read a fixed set of sentences aloud, and the data hook records and saves each sentence. Every later comparison reruns the complete pipeline and only replaces the input with these saved recordings before speech recognition, so the person does not have to read again. Because the sentences are fixed, their text also serves as the reference for the character error rate (CER) of speech recognition. The measurement hook records how long each stage takes for every sentence. The latency is the time from the end of the replayed human recording to the moment Misty actually starts to make sound; this moment is detected by a laptop microphone placed next to Misty.

\paragraph{Baseline and Targets.}
EvoMisty first measures the baseline: a latency of 6.53\,s and a CER of 0.02. The optimization targets are to reduce both as far as possible. The measurement hook splits the latency into the stages of the pipeline: retrieving the recording, speech recognition, reply generation, speech synthesis, and upload until Misty makes sound. The changes that follow address these stages one by one.

\paragraph{What Each Step Changed.}
\Cref{tab:supp-run} lists, in order, changes that improved the results and were kept in the final program, together with the stage that each one targets.


\subsection{Hooks and Changes in All Five Tasks}
\label{sec:supp-opt-hooks}

For each of the five tasks in Table~2 of the main paper, \Crefrange{tab:supp-hooks-ncd}{tab:supp-hooks-mpt} list what the data hook and the measurement hook record, and the main changes that were kept in the final program. Claude Code and Codex are shown side by side.

\begin{table*}[tp]
\caption{Task~\supptaskref{supp:task25}{25}: Naughty-Child Dialogue (\cref{sec:supp-bench-dialogue}). Targets: response latency, CER.}
\label{tab:supp-hooks-ncd}
\supplisttablesetup
\begin{tabularx}{\textwidth}{|l|>{\raggedright\arraybackslash}X|>{\raggedright\arraybackslash}X|}
\hline
 & \textbf{Claude Code} & \textbf{Codex} \\
\hline
Data hook &
  \supphitem{1}{Recordings of a person reading fixed sentences}
  \supphitem{2}{An audio recording of each complete run}
&
  \supphitem{1}{Recordings of a person reading fixed sentences}
  \supphitem{2}{A recording of each turn, from the question to the end of the reply}
  \supphitem{3}{The synthesized reply audio}
\\ \hline
Measurement hook &
  \supphitem{1}{The time of each stage for every sentence, from the end of speech to Misty's first sound}
  \supphitem{2}{The recognized text and Misty's reply}
&
  \supphitem{1}{The time of each stage for every sentence}
  \supphitem{2}{The moments when the user stops speaking and when Misty starts to speak}
  \supphitem{3}{The recognized text}
\\ \hline
Changes kept &
  \supphitem{1}{Speech recognition and speech synthesis run locally on the computer}
  \supphitem{2}{A faster dialogue model is used; the reply is spoken while it is generated, first sentence first}
  \supphitem{3}{Audio is played directly after upload}
  \supphitem{4}{Speech is recorded with the computer's microphone}
&
  \supphitem{1}{Recognition, dialogue, and synthesis all run locally on the computer}
  \supphitem{2}{The reply is spoken while it is generated, first sentence first}
  \supphitem{3}{Misty fetches the reply audio directly from the computer; no upload is needed}
  \supphitem{4}{The reply is prepared in advance as soon as the user pauses}
  \supphitem{5}{The prompt is shortened so that replies are more direct}
  \supphitem{6}{Speech is picked up with the computer's microphone}
\\ \hline
\end{tabularx}
\end{table*}

\begin{table*}[tp]
\caption{Task~\supptaskref{supp:taskN3}{N3}: MistyPilot Emotional Dialogue (\cref{sec:supp-new-harder}). Target: response latency.}
\label{tab:supp-hooks-mped}
\supplisttablesetup
\begin{tabularx}{\textwidth}{|l|>{\raggedright\arraybackslash}X|>{\raggedright\arraybackslash}X|}
\hline
 & \textbf{Claude Code} & \textbf{Codex} \\
\hline
Data hook &
  \supphitem{1}{Recordings of a person reading fixed sentences}
  \supphitem{2}{The audio of each of Misty's replies}
  \supphitem{3}{Room recordings before and after each playback}
&
  \supphitem{1}{Recordings of the user's questions}
  \supphitem{2}{The audio of each of Misty's replies}
  \supphitem{3}{Room recordings while Misty replies}
\\ \hline
Measurement hook &
  \supphitem{1}{The time of each stage for every sentence}
  \supphitem{2}{The moment Misty actually starts to make sound}
  \supphitem{3}{The recognized text}
  \supphitem{4}{The emotion, speaking rate, and motion of each reply}
&
  \supphitem{1}{The recognized text}
  \supphitem{2}{The time from the end of speech to Misty's first sound}
  \supphitem{3}{The time of each stage for every sentence}
\\ \hline
Changes kept &
  \supphitem{1}{Speech recognition runs locally on the computer}
  \supphitem{2}{A faster dialogue model is used}
  \supphitem{3}{Audio is compressed before upload}
  \supphitem{4}{The first sentence is split in two, and the first half is spoken first}
&
  \supphitem{1}{Each sentence of the reply is synthesized as soon as it is complete}
  \supphitem{2}{Speech recognition and speech synthesis run locally on the computer}
  \supphitem{3}{Misty fetches the reply audio directly from the computer; no upload is needed}
  \supphitem{4}{A different audio format is used}
\\ \hline
\end{tabularx}
\end{table*}

\begin{table*}[tp]
\caption{Task~\supptaskref{supp:taskN5}{N5}: Rock-Paper-Scissors (\cref{sec:supp-new-harder}). Target: gesture recognition accuracy.}
\label{tab:supp-hooks-rps}
\supplisttablesetup
\begin{tabularx}{\textwidth}{|l|>{\raggedright\arraybackslash}X|>{\raggedright\arraybackslash}X|}
\hline
 & \textbf{Claude Code} & \textbf{Codex} \\
\hline
Data hook &
  \supphitem{1}{Videos of hand gestures from Misty's camera; some are held out for testing and not used in optimization}
  \supphitem{2}{Labels for each video: gesture, distance, and angle}
&
  \supphitem{1}{Videos of hand gestures from Misty's camera}
  \supphitem{2}{Every frame actually sent to recognition}
\\ \hline
Measurement hook &
  \supphitem{1}{The gesture recognized in each frame and the time taken}
  \supphitem{2}{The final gesture decided for each video}
&
  \supphitem{1}{The final gesture decided for each video, or the reason why none was decided}
  \supphitem{2}{The recognition result and the time taken for each frame}
  \supphitem{3}{The true gesture, checked by a person}
\\ \hline
Changes kept &
  \supphitem{1}{Hands are tracked continuously instead of being detected separately in every frame}
  \supphitem{2}{Duplicate detections of the same hand are merged}
  \supphitem{3}{A learned classifier replaces hand-written rules for gesture classification}
  \supphitem{4}{The decision combines the results of the most recent frames}
&
  \supphitem{1}{The gesture is first judged from the shape of the fingers; the recognizer's result is used only when this fails}
  \supphitem{2}{When the original image gives no result, it is rotated or padded and recognized again}
\\ \hline
\end{tabularx}
\end{table*}

\begin{table*}[tp]
\caption{Task~\supptaskref{supp:taskN6}{N6}: External-Camera Line Following (\cref{sec:supp-new-harder}). Target: lap time.}
\label{tab:supp-hooks-eclf}
\supplisttablesetup
\begin{tabularx}{\textwidth}{|l|>{\raggedright\arraybackslash}X|>{\raggedright\arraybackslash}X|}
\hline
 & \textbf{Claude Code} & \textbf{Codex} \\
\hline
Data hook &
  \supphitem{1}{Video from the overhead camera}
  \supphitem{2}{Misty's position in each frame}
  \supphitem{3}{Readings of the inertial sensor (IMU) and the drive commands sent to Misty}
&
  \supphitem{1}{Each photo taken by the camera}
  \supphitem{2}{The time and duration of each action}
  \supphitem{3}{Video recorded during straight moves}
\\ \hline
Measurement hook &
  \supphitem{1}{Misty's position and the time of each frame, from which the lap time and the distance from the track are computed}
  \supphitem{2}{The time taken by each drive command}
&
  \supphitem{1}{Misty's position at each step, from which the lap time is computed}
  \supphitem{2}{The decision at each step and the duration of each action}
\\ \hline
Changes kept &
  \supphitem{1}{Steering starts early, according to the curvature of the bend ahead}
  \supphitem{2}{Delay compensation also predicts Misty's heading}
  \supphitem{3}{The speed of each part of the lap is planned in advance}
  \supphitem{4}{Heading errors are also corrected on bends}
&
  \supphitem{1}{Straight segments are driven in longer moves, monitored by video along the way}
  \supphitem{2}{The photo taken after a turn is reused for the next step instead of taking a new one}
  \supphitem{3}{A sudden jump in position is re-checked before continuing, instead of aborting}
  \supphitem{4}{Sensor readings decide when a turn has settled, instead of a fixed waiting time}
\\ \hline
\end{tabularx}
\end{table*}

\begin{table*}[tp]
\caption{Task~\supptaskref{supp:taskN7}{N7}: Minimal Pair Therapy (\cref{sec:supp-new-harder}). Targets: pointing-direction accuracy, spoken-word discrimination accuracy.}
\label{tab:supp-hooks-mpt}
\supplisttablesetup
\begin{tabularx}{\textwidth}{|l|>{\raggedright\arraybackslash}X|>{\raggedright\arraybackslash}X|}
\hline
 & \textbf{Claude Code} & \textbf{Codex} \\
\hline
Data hook &
  \supphitem{1}{The audio and Misty's camera images of each trial}
  \supphitem{2}{The correct answers: which card is pointed at and which word is spoken}
&
  \supphitem{1}{Images taken while aligning with the screen}
  \supphitem{2}{The images and audio of each trial}
  \supphitem{3}{The correct answers, confirmed by the user}
\\ \hline
Measurement hook &
  \supphitem{1}{The correct answer and the program's decision for each trial}
  \supphitem{2}{Trials held out for testing are not judged during optimization}
&
  \supphitem{1}{For each trial: the correct answer, the program's decision, and whether it is right}
  \supphitem{2}{The hand detection result in each frame}
  \supphitem{3}{The recognized text}
\\ \hline
Changes kept &
  \supphitem{1}{Hands are searched for only near the cards, in an enlarged view}
  \supphitem{2}{To decide where the finger points, the direction of the index finger is extended forward}
  \supphitem{3}{Each of the two words receives a score, and the higher one is chosen}
  \supphitem{4}{When the sound matches neither word, it is treated as noise and listening continues}
&
  \supphitem{1}{Hands are searched for in views of several angles and ranges; no decision is made when the views conflict}
  \supphitem{2}{Pointing counts only when the index finger is extended and the other fingers are mostly curled}
  \supphitem{3}{To decide where the finger points, the direction of the index finger is extended forward}
  \supphitem{4}{Speech detection replaces a volume threshold for deciding whether someone is speaking}
  \supphitem{5}{A heard word that is not on the cards is judged by which card word it resembles more}
\\ \hline
\end{tabularx}
\end{table*}

\subsection{Optimizing Without EvoMisty}
\label{sec:supp-opt-noevo}
This subsection examines how well a coding agent optimizes a program on its own, without EvoMisty. We use two tasks, Naughty-Child Dialogue and Rock-Paper-Scissors. For each task, Claude Code and Codex, with the models used in the main paper, both start from the program with which Claude Code completed the task in Solve; this is also Claude Code's starting point in Table~2 of the main paper. Each agent receives the optimization targets used with EvoMisty and then works without any intervention from us. The optimized programs are evaluated exactly as in Table~2, with the same test data and procedure. \Cref{tab:supp-noevo} reports the results; for comparison, its With EvoMisty columns repeat Table~2.

\begin{table*}[tp]
\caption{Optimization results with and without EvoMisty.}
\label{tab:supp-noevo}
\supptablesetup
\setlength{\tabcolsep}{5pt}
\begin{tabularx}{\textwidth}{|l|l|l|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|}
\hline
 & & & \multicolumn{2}{c|}{\textbf{Without EvoMisty}} & \multicolumn{2}{c|}{\textbf{With EvoMisty}} \\
\cline{4-7}
\textbf{Task} & \textbf{Metric} & \textbf{Agent} & Before & After & Before & After \\
\hline
Naughty-Child & Response latency (s) $\downarrow$ & Claude Code & 7.41\,$\pm$\,0.70 & 5.28\,$\pm$\,0.86 & 7.41\,$\pm$\,0.70 & \textbf{3.54\,$\pm$\,0.47} \\
\cline{3-7}
Dialogue & & Codex & 7.41\,$\pm$\,0.70 & 5.25\,$\pm$\,0.60$^{*}$ & 7.18\,$\pm$\,1.03 & \textbf{2.06\,$\pm$\,0.25} \\
\cline{2-7}
 & CER $\downarrow$ & Claude Code & 0.053 & 0.022 & 0.053 & \textbf{0.000} \\
\cline{3-7}
 & & Codex & 0.053 & \textcolor{suppred}{0.078} & 0.037 & \textbf{0.000} \\
\hline
Rock-Paper- & Gesture recognition & Claude Code & 0.845 & \textcolor{suppred}{0.763} & 0.845 & \textbf{0.987} \\
\cline{3-7}
Scissors & accuracy $\uparrow$ & Codex & 0.845 & \textcolor{suppred}{0.675} & 0.273 & \textbf{0.874} \\
\hline
\end{tabularx}
\supptablenote{\textcolor{suppred}{Red}: worse than before optimization; \textbf{bold}: best in the row. Time metrics are reported as mean $\pm$ standard deviation. $\downarrow$: lower is better; $\uparrow$: higher is better. $^{*}$\,The optimized program has a bug: in 3 of the 10 turns Misty did not speak, and the latency is computed over the other 7 turns.}
\end{table*}

\paragraph{Claude Code.}
Claude Code prepared its own data for the optimization. For the dialogue task, it wrote 20 sentences, turned them into speech with a speech synthesis model, and then ran the program on the robot to measure the latency. For the gesture task, it downloaded a public dataset of hand-gesture photos from the internet. Neither the speech nor the photos were collected on Misty. After the optimization, the response latency of the dialogue fell from 7.41\,s to 5.28\,s, a smaller reduction than with EvoMisty (3.54\,s); the gesture recognition accuracy was 0.763, which does not exceed below the 0.845 before optimization.

\paragraph{Codex.}
Codex took a static approach rather than a measurement-driven one: it revised the code without collecting any data or running the program on the robot. This matches the observation discussed in Sec.~2.3 of the main paper that agent-authored performance optimizations report explicit performance validation less often than human-authored ones. The optimized programs showed two problems. The dialogue program uploads two audio segments at the same time, but Misty accepts only one upload at a time; as a result, Misty did not speak in 3 of the 10 turns. The rules that decide the gesture were made stricter, and the accuracy fell from 0.845 to 0.675.

\paragraph{What EvoMisty's Optimize Stage Contributes.}
We use the same coding agents and models, and the same optimization targets, with and without EvoMisty. What differs is how a code change is tested and how the test results are used. With EvoMisty, a data hook collects real task data and a measurement hook measures the target metrics. Each change is tested on this data, and the measurements tell the agent what to optimize next.

Without EvoMisty, Codex changed the code but never ran it on the robot, and the program failed on Misty. Claude Code did test on the robot, but it optimized on speech that it had synthesized and on gesture photos from the web, which differ from what the robot hears and sees in the real task. As a result, its latency improved less than with EvoMisty, and its gesture recognition accuracy fell below the baseline.

EvoMisty does not write code changes for the coding agent. It provides feedback, measured on the robot with real task data, that guides the agent's next change.


==> sec/supp_C_evolve.tex <==
\section{Evolve: Skill Distillation and Reuse}
\label{sec:supp-evolve}

In Sec.~4.4.1 of the main paper, EvoMisty distills the optimized program of Naughty-Child Dialogue into skills, and each of the other three dialogue tasks (Math Tutoring, Keyword Story, and Chinese-to-English Translation, \emph{Translation} for short) is solved once without and once with these skills; Table~3 reports the results. The four dialogue tasks follow the same pipeline: speech input, speech recognition, reply generation, speech synthesis, and playback. These steps are called \emph{stages} below. Based on the Skill Library and the final program of each task, this section reports which skills were distilled and how the three tasks use them.

\subsection{Skills Distilled and Reused with Claude Code}
\label{sec:supp-evolve-cc}

\paragraph{Skills Distilled from Naughty-Child Dialogue.}
Distillation produced six skills, which together cover every stage of the dialogue. \Cref{tab:supp-skills-cc} lists them.

\begin{table*}[t]
\caption{Claude Code: distilled skills and their use in the other three dialogue tasks.}
\label{tab:supp-skills-cc}
\supptablesetup
\begin{tabularx}{\textwidth}{|l|>{\raggedright\arraybackslash}X|c|c|c|}
\hline
\textbf{Skill and stage} & \textbf{What it does} & \supptwolinehead{Math}{Tutoring} & \supptwolinehead{Keyword}{Story} & \textbf{Translation} \\
\hline
\suppskillcell{computer\_push\_to\_talk\_mic}{Speech input} & Records push-to-talk audio with the computer microphone; the audio is available as soon as the key is released. & used & used & used \\
\hline
\suppskillcell{sense\_voice\_asr}{Speech recognition} & Recognizes a recording with a local SenseVoice model. & used & used & used \\
\hline
\suppskillcell{streaming\_chat\_reply}{Reply generation} & Keeps the multi-turn history and streams the reply, handing out the first sentence as soon as it is complete. & adapted & -- & -- \\
\hline
\suppskillcell{melo\_tts\_pitched}{Speech synthesis} & Synthesizes pitch-raised Chinese speech with a local MeloTTS model; outputs MP3. & used & used & -- \\
\hline
\suppskillcell{misty\_audio\_player}{Playback} & Uploads audio to Misty, plays it, and waits until playback completes. & used & used & -- \\
\hline
\suppskillcell{misty\_pipelined\_speaker}{Playback} & Synthesizes incoming text segment by segment and plays the segments back to back on Misty; can be interrupted. & used & adapted & -- \\
\hline
\end{tabularx}
\supptablenote{\emph{used}: imported and called, skill code unchanged. \emph{adapted}: not imported; rewritten on the basis of the skill. --: not used.}
\end{table*}

\paragraph{Reuse in the Other Three Dialogue Tasks.}
The three right-hand columns of \Cref{tab:supp-skills-cc} show how the final program of each task uses each skill. The three tasks use the skills selectively, and three cases can be distinguished. First, speech input and speech recognition are the first two stages of the pipeline, and the three tasks have the same needs there. All three tasks use the two corresponding skills, \suppcode{computer\_push\_to\_talk\_mic} and \suppcode{sense\_voice\_asr}, unchanged. Second, the speech synthesis skill \suppcode{melo\_tts\_pitched} synthesizes Chinese speech. Math Tutoring and Keyword Story answer in Chinese and use it together with the two playback skills, \suppcode{misty\_audio\_player} and \suppcode{misty\_pipelined\_speaker}; Translation has to speak English and uses none of the three. Keyword Story has to accompany each segment with expressions and motions when the segment starts to play, so it adapted \suppcode{misty\_pipelined\_speaker}. Third, reply generation is the stage at which the three tasks differ from one another, and no task imports the corresponding skill, \suppcode{streaming\_chat\_reply}, directly. This skill hands out a reply in at most two pieces (the first sentence, then the rest) and always sends the full conversation history. The needs of all three tasks differ from this: Math Tutoring has to explain sentence by sentence, Keyword Story needs an emotion for each segment, and Translation needs no history. Math Tutoring adapted the skill and rewrote the generation part; the other two tasks implemented generation themselves.

\subsection{Skills Distilled and Reused with Codex}
\label{sec:supp-evolve-codex}

\paragraph{Skills Distilled from Naughty-Child Dialogue.}
Distillation produced six skills, covering the stages from speech recognition to playback; audio encoding is a step between speech synthesis and playback. Speech input was not distilled into a skill.

\begin{table*}[t]
\caption{Codex: distilled skills and their use in the other three dialogue tasks.}
\label{tab:supp-skills-codex}
\supptablesetup
\begin{tabularx}{\textwidth}{|l|>{\raggedright\arraybackslash}X|c|c|c|}
\hline
\textbf{Skill and stage} & \textbf{What it does} & \supptwolinehead{Math}{Tutoring} & \supptwolinehead{Keyword}{Story} & \textbf{Translation} \\
\hline
\suppskillcell{sense\_voice\_transcriber}{Speech recognition} & Recognizes a recording with a local SenseVoice model. & used & used & used \\
\hline
\suppskillcell{local\_chat}{Reply generation} & Streams a reply from a local Qwen3-4B model; keeps no history. & used & used & used \\
\hline
\suppskillcell{kokoro\_synthesizer}{Speech synthesis} & Synthesizes Chinese speech with a local Kokoro model and outputs WAV. & used & used & -- \\
\hline
\suppskillcell{speech\_mp3\_encoder}{Audio encoding} & Encodes WAV speech as MP3 and trims the leading silence. & used & used & -- \\
\hline
\suppskillcell{speech\_server}{Playback} & Serves MP3 audio to Misty at a temporary HTTP address on the computer. & indirect & indirect & -- \\
\hline
\suppskillcell{hosted\_audio\_player}{Playback} & Has Misty play the MP3 at that address and waits until playback completes. & used & used & -- \\
\hline
\end{tabularx}
\supptablenote{\emph{used}: imported and called, skill code unchanged. \emph{indirect}: not imported by the task; called by another skill that the task uses. --: not used.}
\end{table*}

\paragraph{Reuse in the Other Three Dialogue Tasks.}
The three right-hand columns of \Cref{tab:supp-skills-codex} show how the final program of each task uses each skill; no task adapted a skill. The three tasks again use the skills selectively, and two cases can be distinguished. First, all three tasks use the speech recognition skill \suppcode{sense\_voice\_transcriber} and the reply generation skill \suppcode{local\_chat} unchanged. The three tasks have the same needs for speech recognition. Their needs for reply generation differ, but \suppcode{local\_chat} only passes the messages to the model and returns its output: it neither splits the reply nor keeps history, and each task handles these itself. Second, the speech synthesis skill \suppcode{kokoro\_synthesizer} synthesizes Chinese speech. Math Tutoring and Keyword Story answer in Chinese and use it together with the encoding and playback skills \suppcode{speech\_mp3\_encoder}, \suppcode{speech\_server}, and \suppcode{hosted\_audio\_player}. Translation has to speak English: it uses none of the four and speaks with Misty's built-in text-to-speech instead. Its version without skills used cloud speech synthesis; this change does not come from a skill.





==> sec/supp_D_benchmark.tex <==
\clearpage     %
\makeatletter\global\@colroom\@colht \global\vsize\@colht\makeatother
\raggedbottom  %
\section{AutoMisty Benchmark Tasks}
\label{sec:supp-benchmark}
The AutoMisty benchmark has 28 tasks in seven categories. Each card below gives the instruction for one task and the success criteria used to judge whether the task is completed.

\subsection{Body Motion}
\label{sec:supp-bench-body}

\begin{supptaskcard}{Task 1}{Raise Hand}
\suppfirstcardpart{Instruction}
``Misty, I need you to raise your \suppph{left/right} hand and then put it back in the initial position.''
\suppcardpart{Success criteria}
\begin{suppenum}
\item Only the \suppph{left/right} hand is raised.
\item After being raised, the hand returns to the initial position.
\end{suppenum}
\end{supptaskcard}

\begin{supptaskcard}{Task 2}{Repeated Hand Raise}
\suppfirstcardpart{Instruction}
``Misty, I need you to raise your \suppph{left/right} hand and put it back in the initial position; this counts as one repetition. Do \suppph{N} repetitions in total.''
\suppcardpart{Success criteria}
\begin{suppenum}
\item Each time, only the \suppph{left/right} hand is raised.
\item Exactly \suppph{N} repetitions are completed, no more and no fewer.
\end{suppenum}
\end{supptaskcard}

\begin{supptaskcard}{Task 3}{Variable-Speed Hand Raise}
\suppfirstcardpart{Instruction}
``Misty, I need you to do the hand-raising motion twice: raise both hands at the same time, then put both back in the initial position at the same time. Do it slowly the first time and fast the second time.''
\suppcardpart{Success criteria}
\begin{suppenum}
\item Both times, both hands are fully raised and put back.
\item The second (fast) time takes clearly less time than the first (slow) time.
\end{suppenum}
\end{supptaskcard}

\begin{supptaskcard}{Task 4}{Turn Head}
\suppfirstcardpart{Instruction}
``Misty, I need you to turn your head to the \suppph{left/right} and then turn it back to the initial position.''
\suppcardpart{Success criteria}
\begin{suppenum}
\item The head turns to the \suppph{left/right}.
\item After turning, the head returns to the initial position.
\end{suppenum}
\end{supptaskcard}

\begin{supptaskcard}{Task 5}{Repeated Head Turn}
\suppfirstcardpart{Instruction}
``Misty, I need you to turn your head to the \suppph{left/right} and back to the initial position; this counts as one repetition. Do \suppph{N} repetitions in total.''
\suppcardpart{Success criteria}
\begin{suppenum}
\item Each time, the head turns to the \suppph{left/right}.
\item Exactly \suppph{N} repetitions are completed, no more and no fewer.
\end{suppenum}
\end{supptaskcard}

\begin{supptaskcard}{Task 6}{Variable-Speed Head Turn}
\suppfirstcardpart{Instruction}
``Misty, I need you to do the head-turning motion twice: turn your head to the left first, then to the right, and finally back to the initial position. Do it slowly the first time and fast the second time.''
\suppcardpart{Success criteria}
\begin{suppenum}
\item Both times, the motion is fully completed in the order left, right, initial position.
\item The second (fast) time takes clearly less time than the first (slow) time.
\end{suppenum}
\end{supptaskcard}

\subsection{Expression and Speech Output}
\label{sec:supp-bench-expression}

\begin{supptaskcard}{Task 7}{Show Expression}
\suppfirstcardpart{Instruction}
``Misty, I need you to show a happy expression on your face screen first, and then switch to an angry expression.''
\suppcardpart{Success criteria}
\begin{suppenum}
\item The happy expression is shown first and the angry expression second.
\item After the switch, the screen shows the new expression and no longer the previous one.
\end{suppenum}
\end{supptaskcard}

\begin{supptaskcard}{Task 8}{Chest Light Color}
\suppfirstcardpart{Instruction}
``Misty, I need you to set your chest LED to \suppph{color} and keep it that color.''
\suppcardpart{Success criteria}
\begin{suppenum}
\item The chest LED is \suppph{color}.
\item After being set, the LED stays \suppph{color}.
\end{suppenum}
\end{supptaskcard}

\begin{supptaskcard}{Task 9}{Variable-Speed Self-Introduction}
\suppfirstcardpart{Instruction}
``Misty, I need you to say this self-introduction twice: `Hello, I am Misty, your little friend.' Say it slowly the first time and fast the second time.''
\suppcardpart{Success criteria}
\begin{suppenum}
\item The sentence is spoken in full both times.
\item The speaking rate of the second (fast) time is clearly higher than that of the first (slow) time.
\end{suppenum}
\end{supptaskcard}

\subsection{Multimodal Performance}
\label{sec:supp-bench-multimodal}

\begin{supptaskcard}{Task 10}{Tell \textit{The Three Little Pigs}}
\suppfirstcardpart{Instruction}
``Misty, I need you to tell the story of \textit{The Three Little Pigs} once, with facial expressions and sound effects while you tell it.''
\suppcardpart{Success criteria}
\begin{suppenum}
\item The whole story is told, with all the main plot points.
\item The telling is accompanied by facial expressions and sound effects.
\end{suppenum}
\end{supptaskcard}

\begin{supptaskcard}{Task 11}{Compose and Recite a Poem}
\suppfirstcardpart{Instruction}
``Misty, I need you to compose a poem on the theme `I love research' and then recite it in full. While reciting, use arm movements together with at least one of facial expressions or lights.''
\suppcardpart{Success criteria}
\begin{suppenum}
\item The poem is on the theme `I love research' and is recited in full.
\item The recitation is accompanied by arm movements and by at least one of facial expressions or lights.
\end{suppenum}
\end{supptaskcard}

\begin{supptaskcard}{Task 12}{Rock Dance}
\suppfirstcardpart{Instruction}
``Misty, I need you to perform a rock-style dance, using arm movements, facial expressions, lights, and sound together to express the rhythm.''
\suppcardpart{Success criteria}
\begin{suppenum}
\item A coherent dance is completed, with clearly visible body movements.
\item The movements are accompanied by facial expressions, lights, and sound.
\end{suppenum}
\end{supptaskcard}

\begin{supptaskcard}{Task 13}{Comfort}
\suppfirstcardpart{Instruction}
``Misty, I am feeling very sad right now, and I need you to comfort me: say warm, comforting words, accompanied by caring facial expressions, movements, and sound.''
\suppcardpart{Success criteria}
\begin{suppenum}
\item Misty says comforting words that respond to the sadness.
\item The words are accompanied by caring facial expressions, movements, and sound.
\end{suppenum}
\end{supptaskcard}

\begin{supptaskcard}{Task 14}{Drink-Water Reminder}
\suppfirstcardpart{Instruction}
``Misty, I need you to set a timer for \suppph{duration}. As soon as the time is up, remind me to drink water, with at least one of facial expressions, lights, or arm movements. Then keep reminding me, and stop only when I press and hold your front bumper.''
\suppcardpart{Success criteria}
\begin{suppenum}
\item When the \suppph{duration} timer ends, Misty reminds the person to drink water, with at least one of facial expressions, lights, or arm movements.
\item Misty keeps reminding while the person is not holding the bumper, and the reminders stop once it is held.
\end{suppenum}
\end{supptaskcard}

\subsection{Touch Interaction}
\label{sec:supp-bench-touch}

\begin{supptaskcard}{Task 15}{Head-Touch Emotional Reaction}
\suppfirstcardpart{Instruction}
``Misty, I need you to react emotionally when your head is touched: when I touch the top of your head, act happy and excited; when I touch the back of your head, act angry. Every reaction must use your facial expression, chest LED, arm movements, and speech at the same time.''
\suppcardpart{Success criteria}
\begin{suppenum}
\item After the person touches the top of the head, Misty shows happiness or excitement, and the person can see or hear this emotion.
\item After the person touches the back of the head, Misty shows anger, and the person can see or hear this emotion.
\item Every reaction uses facial expression, chest LED, arm movements, and speech at the same time.
\end{suppenum}
\end{supptaskcard}

\begin{supptaskcard}{Task 16}{Head-Touch Pikachu}
\suppfirstcardpart{Instruction}
``Misty, I need you to imitate Pikachu's cry once, `Pika Pika', after I touch the front of your head. When I have not touched it, do not make the cry.''
\suppcardpart{Success criteria}
\begin{suppenum}
\item After the person touches the front of the head, Misty makes Pikachu's cry.
\item Without a touch, Misty does not make the cry.
\end{suppenum}
\end{supptaskcard}

\begin{supptaskcard}{Task 17}{Head-Touch Countdown Photo}
\suppfirstcardpart{Instruction}
``Misty, after I touch the front of your head, I need you to count down `3, 2, 1' in order, then take a photo with your camera and save it to the computer, and finally do a cute action (at least one of waving your arms, changing your expression, or saying a sentence).''
\suppcardpart{Success criteria}
\begin{suppenum}
\item After the person touches the front of the head, Misty starts the countdown and says 3, 2, 1 in order.
\item After the countdown, Misty takes a photo and saves it to the computer; the file opens normally and shows the scene in front of Misty's camera.
\item After the photo is saved, Misty does a cute action (at least one of waving its arms, changing its expression, or saying a sentence).
\end{suppenum}
\end{supptaskcard}

\subsection{Voice Commands and Question Answering}
\label{sec:supp-bench-voice}

\begin{supptaskcard}{Task 18}{Greeting}
\suppfirstcardpart{Instruction}
``Misty, I need you to keep listening to me. Whenever I say `Hello Misty', say in full: `Hello, I am Misty, your companion.' Then keep listening, and respond again when I say `Hello Misty' again. When I say anything else, do not respond.''
\suppcardpart{Success criteria}
\begin{suppenum}
\item After the person says `Hello Misty', Misty says in full: `Hello, I am Misty, your companion.'
\item Without restarting the program, each time a response has finished and the person says `Hello Misty' again, Misty responds.
\item When what the person says is not `Hello Misty', Misty does not respond.
\end{suppenum}
\end{supptaskcard}

\begin{supptaskcard}{Task 19}{Voice-Controlled Chest Light Color}
\suppfirstcardpart{Instruction}
``Misty, I need you to listen for a color. After I say one of the color names red, green, blue, yellow, or purple, change your chest LED to that color. When what I say contains no color name, or when I say nothing, keep the LED unchanged.''
\suppcardpart{Success criteria}
\begin{suppenum}
\item After the person says one of the color names red, green, blue, yellow, or purple, the LED changes to that color, and the person judges by eye that the color matches.
\item When what the person says contains no color name, or when nobody speaks, the LED stays unchanged.
\end{suppenum}
\end{supptaskcard}

\begin{supptaskcard}{Task 20}{Voice-Triggered Photo}
\suppfirstcardpart{Instruction}
``Misty, I need you to keep listening to me. Whenever I say `cheese', take a photo of the current view with your camera and save it to the computer: save only one photo each time, and keep the earlier photos. Then keep listening, so that I can say `cheese' again to trigger another photo. When I say anything else or say nothing, do not take a photo.''
\suppcardpart{Success criteria}
\begin{suppenum}
\item After the person says `cheese', Misty captures a photo of the current camera view.
\item The photo can be found on the computer, the file opens normally, and its content matches the scene in front of the camera at the time of this trigger.
\item Each valid trigger saves only one photo; without restarting the program, a photo can be triggered again, and the earlier photos are still kept.
\item When the person says something else or stays silent, no photo is triggered.
\end{suppenum}
\end{supptaskcard}

\begin{supptaskcard}{Task 21}{Voice-Controlled Video Recording}
\suppfirstcardpart{Instruction}
``Misty, I need you to keep listening for my voice commands. After I say `go', start recording the camera view; after I say `stop', stop recording and save the video. When I say anything else or say nothing, do not start recording and do not stop recording.''
\suppcardpart{Success criteria}
\begin{suppenum}
\item After the person says `go', recording of Misty's camera view starts.
\item After the person says `stop', the recording stops and the video is saved; the file plays normally.
\item When the person says something else or stays silent, neither start nor stop is triggered.
\end{suppenum}
\end{supptaskcard}

\begin{supptaskcard}{Task 22}{Direction Memory Game}
\suppfirstcardpart{Instruction}
``Misty, I need you to play a direction memory game with me. In each round, first indicate one direction, left or right, with body language (for example, by raising your right hand) and say `Remember the direction I am indicating'; after the motion ends, ask me which direction it was; after I answer, say whether I was right or wrong.''
\suppcardpart{Success criteria}
\begin{suppenum}
\item In each round, Misty indicates one direction (left or right) with body language and prompts the person to remember it.
\item Misty asks the person which direction it was.
\item After the person answers, Misty states its judgment, and the judgment is correct: a right answer is called right and a wrong answer is called wrong.
\end{suppenum}
\end{supptaskcard}

\subsection{Visual Understanding}
\label{sec:supp-bench-visual}

\begin{supptaskcard}{Task 23}{Read a Sign}
\suppfirstcardpart{Instruction}
``Misty, I will hold a sign with English text in front of your camera. Whenever I say `now', read out in full the text on the sign I am currently holding. When I have not said `now', do not read.''
\suppcardpart{Success criteria}
\begin{suppenum}
\item Each time the person finishes saying `now', Misty starts reading the text on the sign currently being held.
\item Misty reads out everything on the sign.
\item When the person does not say `now', Misty does not read the sign.
\end{suppenum}
\end{supptaskcard}

\begin{supptaskcard}{Task 24}{Head-Touch Photo Description}
\suppfirstcardpart{Instruction}
``Misty, after I touch the front of your head, I need you to take a photo of the current scene with your camera and then say what is in the photo. The description must be based on this photo and get the main objects or the scene right.''
\suppcardpart{Success criteria}
\begin{suppenum}
\item After the person touches the front of Misty's head, Misty captures a photo taken after this touch, showing the current scene in front of Misty's camera.
\item Misty says its description of the photo in full.
\item The description is based on this photo and correctly names the main objects or the scene.
\end{suppenum}
\end{supptaskcard}

\subsection{Spoken Dialogue}
\label{sec:supp-bench-dialogue}

\begin{supptaskcard}[supp:task25]{Task 25}{Naughty-Child Dialogue}
\suppfirstcardpart{Instruction}
``Misty, I need you to play a naughty, curious child and keep up a conversation with me in Chinese. Each time I finish a sentence, answer in Chinese: the answer must be on topic and said in full, with simple words and a curious or naughty tone. You are a child throughout the conversation, and you must remember what we said earlier.''
\suppcardpart{Success criteria}
\begin{suppenum}
\item Each time the person finishes a sentence, Misty answers in Chinese, and the answer is on topic and said in full.
\item When the person asks `Are you a child?', Misty can express that it is a child.
\item The answers sound like a child's: simple words and a liking for short sentences.
\item The answers connect to the earlier conversation: when the person asks `What was the first question I just asked you?', Misty answers correctly.
\end{suppenum}
\suppcardpartnote{Optimization target}{(added in this work; not part of the AutoMisty task)}
(1) Response latency: the time from the end of the person's utterance to the moment Misty starts speaking; lower is better. (2) Character error rate (CER) of the system's transcription of the person's speech; lower is better.
\end{supptaskcard}

\begin{supptaskcard}{Task 26}{Math Tutoring}
\suppfirstcardpart{Instruction}
``Misty, I will say a simple math problem in Chinese. After I finish, explain in Chinese how to solve it: give at least one intermediate step, and say the correct answer at the end.''
\suppcardpart{Success criteria}
\begin{suppenum}
\item After the person finishes the problem, Misty explains in Chinese.
\item The final answer is correct.
\item The explanation has at least one intermediate step that is correct and consistent with the problem, rather than only stating the answer.
\end{suppenum}
\end{supptaskcard}

\begin{supptaskcard}{Task 27}{Keyword Story}
\suppfirstcardpart{Instruction}
``Misty, I will say a keyword. After I finish, make up an interesting story around this keyword. Accompany the telling with facial expressions and arm movements.''
\suppcardpart{Success criteria}
\begin{suppenum}
\item After the person says the keyword, Misty starts telling a story.
\item The story is generated from the keyword given this time, and its content revolves around the keyword.
\item The telling is accompanied by facial expressions and arm movements.
\end{suppenum}
\end{supptaskcard}

\begin{supptaskcard}{Task 28}{Chinese-to-English Translation}
\suppfirstcardpart{Instruction}
``Misty, I will say a sentence in Chinese. After I finish, translate it into English and say the translation in full in English.''
\suppcardpart{Success criteria}
\begin{suppenum}
\item After the person finishes a sentence in Chinese, Misty says the translation in full in English.
\item The meaning of the translation is consistent with the original sentence.
\end{suppenum}
\end{supptaskcard}


==> sec/supp_E_newtasks.tex <==
\section{New Tasks}
\label{sec:supp-newtasks}

The seven new tasks test whether a system can go beyond what a hand-designed framework anticipates; each card below gives the description of one task, its success criteria, and, where the task has them, its optimization targets.

\subsection{Extensions of Benchmark Tasks}
\label{sec:supp-new-extensions}

\begin{supplongtaskcard}{Task N1}{Original-Voice Pikachu}
\suppfirstcardpart{Task}
After the person touches the front of Misty's head, Misty plays Pikachu's cry, `Pika Pika', and at the same time shows a randomly chosen Pikachu image on its screen. Both the sound and the images are material from existing Pikachu works found on the web; an imitated cry and AI-generated images or animations are not used.
\suppcardpart{Success criteria}
\begin{suppenum}[midpenalty=10000]
\item After the person touches the front of Misty's head, Misty starts playing Pikachu's cry.
\item The cry is original audio from a Pikachu work; it is not imitated or synthesized by the system.
\item While the cry is playing, the screen shows, in sync, a Pikachu image or animation chosen at random from the existing image material.
\end{suppenum}
\end{supplongtaskcard}

\begin{supplongtaskcard}{Task N2}{Face-Tracking Recording}
\suppfirstcardpart{Task}
The program keeps listening for voice commands. After the person says `go', Misty starts recording the camera view and keeps tracking the person's face by rotating left and right, so that the face stays as close to the center of the frame as possible. After the person says `stop', Misty stops recording and saves the video.
\suppcardpart{Success criteria}
\begin{suppenum}
\item After the person says `go', recording of Misty's current camera view starts.
\item During recording, Misty rotates left and right as the position of the face changes, keeping the face as close to the center of the frame as possible.
\item Recording continues until the person says `stop'.
\item The saved video can be found on the computer, the file plays normally, and its content includes the changes that actually happened in front of the camera during recording.
\item Without a start command there is no recording; other speech and silence trigger neither start nor stop.
\item Without restarting the program, another recording can be made with `go' and `stop'; the previous video is still kept.
\end{suppenum}
\end{supplongtaskcard}

\subsection{Harder New Tasks}
\label{sec:supp-new-harder}

\begin{supplongtaskcard}[supp:taskN3]{Task N3}{MistyPilot Emotional Dialogue}
\suppfirstcardpart{Task}
Read the source code of MistyPilot in its GitHub repository, extract and reuse its emotional expression mechanism, and build an emotional dialogue system for Misty that runs on its own and supports continuous multi-turn spoken interaction. The core goal is that Misty understands the user's speech, replies naturally in context, and expresses itself through emotional speech and motion.

\suppcardhead{Core functions}
\textbf{1. Reuse MistyPilot's emotional expression mechanism.} Keep MistyPilot's original emotional expression logic as completely as possible, including:
\begin{suppdash}
\item Prompts: the prompts for generating and expressing emotions.
\item Speech: the parameters for each emotion, such as tone, intonation, and speaking rate.
\item Motion: the robot motions that match each emotion.
\item Coordination of speech and motion: speech and motion are combined by the original mechanism, for natural emotional expression.
\end{suppdash}

\textbf{2. Continuous multi-turn spoken dialogue.} The system must form a complete interaction loop:
\begin{suppparen}
\item Listen to the user: capture the speech and recognize it as text.
\item Generate the reply and the emotion: from the current input and the dialogue context, generate a natural reply and choose a suitable emotion.
\item Express the emotion: call the extracted MistyPilot mechanism so that Misty responds with the corresponding speech and motion.
\item Continue the dialogue: keep the necessary dialogue context and wait for the user's next input, so that the exchange can go on.
\end{suppparen}

\textbf{3. Keypad control.} The whole dialogue system is controlled with the up, middle, and down keys of a small keypad: holding a key starts an action and releasing it ends the action.
\begin{suppdash}
\item Up key, speech input: holding the up key starts recording the user's speech, and releasing it ends the recording. The system then recognizes the speech, generates the reply and the emotion, and has Misty start the corresponding speech and motion.
\item Middle key, interrupting the reply: pressing the middle key immediately interrupts Misty's current speech and the motion that goes with it, cancels the part of the reply that has not been performed, and returns to waiting for user input.
\item Down key, exiting the program: pressing the down key ends the whole dialogue system, stops the current speech, motion, and related tasks, and releases the resources safely.
\end{suppdash}

Interaction principle: the user decides when to speak with the up key, can interrupt the robot at any time with the middle key, and exits with the down key. After an interruption the existing dialogue context is kept, and the conversation can continue.

\textbf{4. Minimal dependencies.} Keep only the functions needed for emotional dialogue; do not port the full MistyPilot framework.
\begin{suppdash}
\item Remove unrelated functions: fast thinking, long-term memory, instruction parsing, model switching, and similar functions are not needed.
\item Keep modules only as needed: if Misty can still hold an emotional multi-turn spoken dialogue after a module is removed, the module is not kept.
\item Keep the necessary context: keep the context needed for multi-turn dialogue, but do not bring in MistyPilot's separate memory system.
\item Adjust the LLM prompts accordingly: any LLM prompt must be checked and adjusted so that it is consistent with the functions, the workflow, and the actual code of the reduced system. Remove dependencies on deleted modules and unrelated instructions, while keeping the original emotional expression prompts and their core mechanism as far as possible.
\end{suppdash}

Core principle: the code and the LLM prompts must be consistent. A prompt must not ask for a function that has been removed.

\textbf{5. Standalone operation.} Put the extracted functions and the necessary dependencies into a separate folder, so that the system does not depend on any other code, configuration, or runtime environment of the MistyPilot repository.
\suppcardrule
\suppfirstcardpart{Success criteria}
\begin{suppenum}
\item Consistency of emotional expression: within the hardware constraints of the project, MistyPilot's original emotional expression logic is fully kept, including the prompts, the tone, intonation, and speaking rate, and the mechanism that coordinates motion.
\item Completeness of multi-turn dialogue: the system generates replies from the dialogue context, chooses a fitting emotion by itself, and expresses it through speech and motion.
\item Correctness of interaction control: the up key reliably starts a turn; the middle key immediately interrupts the robot's current reply; the down key exits the program safely. An interruption does not make the system hang or prevent the dialogue from continuing.
\item System consistency: the prompts and the motion parameters for emotional expression stay consistent with those of MistyPilot.
\item Independence: all emotional dialogue functions work without the original MistyPilot repository.
\end{suppenum}
\suppcardrule
\suppfirstcardpart{Optimization target}
While all core emotional interaction functions are kept, the system may choose cloud models, local models, or a mix by itself, and the optimization method is not restricted. The metric to optimize is the end-to-end response latency: the time from the user releasing the key (the end of the speech input) to Misty actually starting to speak; lower is better.
\end{supplongtaskcard}

\begin{supplongtaskcard}{Task N4}{Gamepad Teleoperation}
\suppfirstcardpart{Task}
Connect a gamepad and, in one program, implement Misty's driving, arm control, hold-to-record and release-to-send speech, local video recording, and a live display of the camera view and the running state.

\suppcardhead{Functional requirements}
\textbf{1. Direction control with continuous acceleration.} The up, down, left, and right buttons of the D-pad drive Misty forward, backward, turning left in place, and turning right in place. While the same direction is held, the speed rises gradually from a low initial speed and stays at the set maximum once it is reached; releasing the button stops Misty immediately. Pressing again or switching direction starts again from the low initial speed. The initial speed, the maximum speed, and the acceleration time are configurable.

\textbf{2. Two sticks mapped to arm positions.} The vertical axes of the left and right sticks control the left and right arms. The stick position is mapped stably to a target angle within the valid range of motion of the corresponding arm, and the arm holds the target position after reaching it. When a stick returns to center, the arm returns to the mapped middle position. The two sticks can be used independently or at the same time.

\textbf{3. Live view and local console.} Misty's camera view is shown continuously, with the correct orientation and a normal aspect ratio, and it follows the scene promptly, without a backlog of old frames causing a visible delay. The resolution, frame rate, and image quality of the video are not fixed and may be adjusted to the device and the network; timely updates of the view during teleoperation have priority. The console shows the connection state of the robot and of the gamepad, the driving direction and speed, the target positions of both arms, the state of the voice function, and the recording state and the save location. The state of the voice function must distinguish `recording', `sending', `playing', and `idle'.

\textbf{4. Hold A to record, release to send the whole utterance.} While the A button is held, the operator's speech is recorded with the computer's microphone; releasing the A button ends the recording and sends the complete recording to Misty for playback.

\textbf{5. Hold Y to record video and save it locally.} While the Y button is held, the camera stream is recorded; releasing the button ends the recording, which is saved automatically to the local recording folder. Each hold produces a separate video, named with a timestamp so that existing files are not overwritten.
\suppcardrule
\suppfirstcardpart{Success criteria}
Verified within the same program:
\begin{suppdash}
\item All four directions are correct; holding accelerates and releasing stops.
\item The two sticks control their corresponding arms.
\item The preview has the correct orientation and follows the scene promptly.
\item Holding A records, and after release Misty plays the whole utterance.
\item Holding Y records video, which is saved automatically on release and plays normally.
\end{suppdash}
\end{supplongtaskcard}

\begin{supplongtaskcard}[supp:taskN5]{Task N5}{Rock-Paper-Scissors}
\suppfirstcardpart{Task}
Misty plays rock-paper-scissors with the user. Misty recognizes the user's gesture with its camera, shows its own move on its screen, and reacts to the result of the game with emotional, humorous speech and motion. Several rounds are played in a row, and the total score and the final winner are announced at the end.

\suppcardhead{Functional requirements}
\textbf{1. Gesture recognition.} Recognize the user's rock (a fist), scissors (index and middle fingers extended), and paper (an open palm) with Misty's camera, for the left and the right hand. If no hand is detected, the gesture is unclear, or several hands appear, ask the user to play again; do not guess and do not score.

\textbf{2. Robot move.} At the start of each round, Misty randomly chooses one move and locks it. Only after the countdown has ended and the user's move has been recognized does Misty show its choice on the screen; the choice must not be changed according to the user's gesture.

\textbf{3. Game flow.} Misty says `Ready? Rock, paper, scissors!', and the user shows a move at the end of the call and holds it briefly. Once the gesture is confirmed to be stable, the system judges it once; if recognition fails, the user is asked to try again, and the robot move already locked for this round is kept.

\textbf{4. Result feedback.} The result follows the rules that rock beats scissors, scissors beats paper, and paper beats rock. Misty reacts with emotional speech and motion that fit the result, for example happy when it wins, dejected when it loses, and playful on a draw, and updates the score.

\textbf{5. Consecutive rounds.} By default, 3 valid rounds are played. The winner of a round gets 1 point; a draw gives no point but counts as a valid round; a failed recognition does not count as a round. At the end of the game the total score and the final winner are announced. The user can end the game early.
\suppcardrule
\suppfirstcardpart{Success criteria}
\begin{suppenum}
\item The three gestures rock, paper, and scissors are recognized.
\item In each round, Misty locks its own move first and then recognizes the user's gesture.
\item The results and the scoring are correct, and the total score and the final winner are announced at the end.
\item When recognition fails, a retry is requested and the score is not affected.
\item Misty's speech and motion are emotionally expressive and fit the current result of the game, so that the interaction is natural and fun.
\end{suppenum}
\suppcardrule
\suppfirstcardpart{Optimization target}
Gesture recognition accuracy: raise the accuracy with which the system recognizes the three gestures rock, paper, and scissors.
\end{supplongtaskcard}

\begin{supplongtaskcard}[supp:taskN6]{Task N6}{External-Camera Line Following}
\suppfirstcardpart{Task}
A clear gray loop track is laid out on the floor, and a purple line marks the start and the finish.

With an external camera as the navigation camera, design the track recognition and the line-following control so that Misty recognizes the gray track and keeps driving along the loop. While driving, the center of the robot's base should stay above the track as far as possible; when Misty deviates, it must adjust its heading by itself and return to the track.
\suppcardpart{Success criteria}
\begin{suppenum}
\item Automatic correction: when Misty deviates while driving, it adjusts its heading by itself and returns to the track.
\item One full lap: Misty completes one lap, with the purple line as the start and the finish.
\end{suppenum}
\suppcardpart{Optimization target}
Lap time, to be minimized: provided that Misty follows the line stably, corrects itself automatically, and completes a full lap, shorten the time from the first crossing of the purple line to the next crossing of the purple line after a full lap.
\end{supplongtaskcard}

\begin{supplongtaskcard}[supp:taskN7]{Task N7}{Minimal Pair Therapy}
\suppfirstcardpart{Task}
Misty introduces the two words on the screen, guides the child to identify each word, to point to a card, and to say the word, and then gives feedback according to whether the card the child actually points to matches the independently recognized word. The teaching web page is \suppcode{flashcards\_site/flashcards\_local.html}.

\suppcardhead{Part 1. Parse and prepare all teaching material in advance}
Before teaching starts, all word pairs planned for the session are prepared; during teaching, the saved material is switched in a fixed order.

\textbf{1. Prepare all word pairs.} Each click on the \textbf{Create} button of the web page generates one word pair. First decide how many word pairs the session needs, then click \textbf{Create} repeatedly and note the pair generated each time, until there are enough; if a pair is repeated or the generation fails, click again.

\textbf{2. Organize the cards and the teaching order.} Save the following information for each word pair: the words, the target phonemes, the voicing labels, the pictures, and the left and right positions. Fix the teaching order, and make sure that the same cards can be shown again during teaching.

\textbf{3. Prepare all lines.} This task is for a special-education setting, so the robot's speech must follow the fixed lines S1--S19 below. Generate the pronunciation cues of the left and the right card by the rules below, fill them into the corresponding places of S1--S19, and prepare, for the two words of each pair, every feedback line that might be needed.

\textbf{4. Generate all speech and expression.} Generate and save the speech of all lines in advance; generic lines are prepared only once. The prepared material is played during teaching. Emotional expression only changes the way of speaking; it does not rewrite the lines.

\textbf{5. Confirm that the material is ready.} Check that all cards can be shown normally, that the lines and the speech are complete, and that the lines and the speech match their cards. When everything is ready, show the first pair of cards, and then go on to screen alignment and teaching.

\suppcardhead{Rules for generating the pronunciation cues}
For the left and the right card separately, follow the steps below, keeping the cue wording of the earlier version of the task, to produce \suppcode{left\_therapy} and \suppcode{right\_therapy}.

\textbf{Step 1: read the card.} Read the word, the target phoneme, and the voicing label from the current card, for example \suppcode{pig}, \suppcode{/p/}, \suppcode{voiceless}. Use the target phoneme marked on the web page; do not guess it from the first letter of the word.

\textbf{Step 2: choose the cue words.} By the voicing label: \suppcode{voiceless}\,\supparr\,\suppcode{quiet}; \suppcode{voiced}\,\supparr\,\suppcode{loud}. By the target phoneme: \suppcode{/p/}\,\supparr\,\suppcode{pa}; \suppcode{/b/}\,\supparr\,\suppcode{ba}; \suppcode{/r/}\,\supparr\,\suppcode{rah}; \suppcode{/s/}\,\supparr\,\suppcode{sa}; \suppcode{/k/}\,\supparr\,\suppcode{ka}; \suppcode{/g/}\,\supparr\,\suppcode{ga}; \suppcode{/l/}\,\supparr\,\suppcode{la}.

\textbf{Step 3: form the cue.} Join \suppcode{quiet} or \suppcode{loud}, the cue syllable, and \suppcode{sound} into one phrase. The cue of the left card is \suppcode{left\_therapy} and the cue of the right card is \suppcode{right\_therapy}; they are used to fill in the lines below.

\textbf{Step 4: fill in the lines and generate the speech.} Fill each word and its cue into the corresponding places of S3, S9, S10, S11, and S16, confirm the content, and then generate all the speech together.

\textbf{Example.} The left card is \suppcode{pig} and the right card is \suppcode{big}.
\begin{suppdash}
\item Left card: the word is \suppcode{pig}, the target phoneme on the web page is \suppcode{/p/}, and the voicing label is \suppcode{voiceless}, which gives \suppcode{left\_therapy = "quiet pa sound"}.
\item Right card: the word is \suppcode{big}, the target phoneme on the web page is \suppcode{/b/}, and the voicing label is \suppcode{voiced}, which gives \suppcode{right\_therapy = "loud ba sound"}.
\end{suppdash}

Filled into S3, the complete line is: `Pig, with the quiet pa sound, and big, with the loud ba sound.'

In a line, \suppvar{word} and \suppvar{therapy} must refer to the same word. If a phoneme, a voicing label, or the cue syllable is unclear, confirm the correct content first, and only then go on preparing the material.

\suppcardhead{Fixed lines S1--S19}
Variables:
\begin{suppdash}
\item \suppvar{left}, \suppvar{right}: the words on the left and the right card.
\item \suppvar{left\_therapy}, \suppvar{right\_therapy}: the pronunciation cues of the left and the right card.
\item \suppvar{word}: in word identification, the word that is asked for; in saying practice, the word the child actually points to.
\item \suppvar{therapy}: the pronunciation cue of the current word.
\item \suppvar{other\_therapy}: the pronunciation cue of the other word.
\end{suppdash}

`Left' and `right' refer to the positions of the cards, not to the hand the child uses. The emotion settings below apply to robots that can express emotions.

\suppcardgroup{Opening and introduction of the word pair}
\suppsline{S1 Opening.}{``Hi! I'm Misty!''}{Emotion: Neutral. Used: at the opening of the first word pair.}

\suppsline{S2 Introducing the activity.}{``Today I will be showing you two words.''}{Emotion: Neutral. Used: for the first word pair, right after S1.}

\suppsline{S3 Introducing the current word pair.}{``\suppvar{left}, with the \suppvar{left\_therapy}, and \suppvar{right}, with the \suppvar{right\_therapy}.''}{Emotion: Neutral. Used: for the introduction of every word pair.}

\suppcardgroup{Word identification: question and feedback}
\suppsline{S4 Identification question.}{``Now, can you point and show me which one is \suppvar{word}?''}{Emotion: Neutral. Used: for the identification question; prepared for the left and the right word separately.}

\suppsline{S5 First successful identification.}{``Well done!''}{Emotion: Excitement. Used: for the first successful identification in the current pair.}

\suppsline{S6 Later successful identification, or end of the pair.}{``Great job!''}{Emotion: Excitement. Used: for later successful identifications in the current pair, or as encouragement when the practice of the whole pair ends.}

\suppsline{S7 Asking again after the first wrong pointing.}{``Incorrect. Please try again. Which one is \suppvar{word}?''}{Emotion: Distress. Used: when the first identification attempt points to the wrong card; asks for the current target word again.}

\suppcardgroup{Saying practice and feedback}
\suppsline{S8 Entering saying practice.}{``Now it's your turn. Can you point to a picture and say the word out loud?''}{Emotion: Neutral. Used: after both words have been identified correctly, to enter saying practice.}

\suppsline{S9 Current word matches; continue with the other word.}{``Good job. You said \suppvar{word} with the \suppvar{therapy}. Now, please try the other word.''}{Emotion: Pleasure. Used: when the current word matches, this word has no earlier mismatch, and the other word is not finished yet.}

\suppsline{S10 Current word matches; the other word is finished.}{``Good job. You said \suppvar{word} with the \suppvar{therapy}.''}{Emotion: Pleasure. Used: when the current word matches, this word has no earlier mismatch, and the other word is already finished.}

\suppsline{S11 Successful retry after the first error.}{``Well done! You said it differently this time. You used the \suppvar{therapy} instead of the \suppvar{other\_therapy}.''}{Emotion: Excitement. Used: when the current word is retried after its first error and matches this time.}

\suppsline{S12 Leading to the other word.}{``Now, please try the other word.''}{Emotion: Pleasure. Used: appended after S11 or S16 when the other word is not finished yet; also used to lead the child to the other word when the child chooses a word that is already finished.}

\suppsline{S13 First error on the left word.}{``Good try! Let's try saying \suppvar{left} one more time.''}{Emotion: Pleasure. Used: when the child points to the left card, the system recognizes the right word, and this is the first error counted for the left word; encourages a retry.}

\suppsline{S14 First error on the right word.}{Two segments, played one after the other: ``Good try!'' and ``Let's try saying \suppvar{right} one more time.''}{Emotion: Pleasure. Used: when the child points to the right card, the system recognizes the left word, and this is the first error counted for the right word; encourages a retry. The two segments are played back to back, and no answer is collected between them.}

\suppsline{S15 Unclear pointing.}{``Can you point to a picture first, and then say the word?''}{Emotion: Neutral. Used: in saying practice, when the pointing of the finger is unclear.}

\suppsline{S16 Second error on the current word.}{``Good try! Listen: \suppvar{word}, with the \suppvar{therapy}.''}{Emotion: Pleasure. Used: at the second error counted for the current word; demonstrates the correct reading and the pronunciation cue, ends the practice of this word, and records it as not passed.}

\suppsline{S17 Not heard clearly.}{``I didn't hear that. Can you say it again?''}{Emotion: Neutral. Used: in saying practice, when nothing is heard or the word the child said cannot be determined.}

\suppcardgroup{Switching pairs and ending}
\suppsline{S18 Switching to the next pair.}{``Let's do the next one.''}{Emotion: Neutral. Used: when the current pair is finished and the next pair is about to be shown.}

\suppsline{S19 Ending the session.}{``That's all for today. Thank you for practicing with me. Bye-bye!''}{Emotion: Pleasure. Used: at the normal end, or when the session ends after two consecutive unfinished identifications.}

Versions to prepare:
\begin{suppdash}
\item S4, S7, S9, S10, S11, S16: prepare a version for each of the two words.
\item S3, S13, S14: fill in the content of the current word pair.
\item All other lines: prepared as generic lines.
\item S14: keep the two speech segments; they are played back to back, and no answer is collected between them.
\end{suppdash}

\suppcardhead{Part 2. Let Misty align itself with the screen}
Misty is placed at a safe, fixed position. It must turn its base by itself and adjust its position and angle, so that the camera clearly sees the screen and the child's finger. Misty must find the best viewing angle by itself, to reduce the rate of misjudgments.

\suppcardhead{Part 3. Carry out the teaching flow}
\textbf{1. Opening and introduction.}
\begin{suppdash}
\item First word pair: play S1\,\supparr\,S2\,\supparr\,S3 in order.
\item Later word pairs: play only S3.
\end{suppdash}

\textbf{2. Identifying the left word.} Play S4(left), wait for the child to point to a card, and act on the result:
\begin{suppdash}
\item Correct: play S5 and go on to identifying the right word.
\item Wrong on the first attempt: play S7(left) and let the child try once more.
\item Unclear pointing or no response on the first attempt: replay S4(left) and let the child try once more.
\item Still not correct on the second attempt: play S19 and end the session.
\end{suppdash}

\textbf{3. Identifying the right word.} Play S4(right), wait for the child to point to a card, and act on the result:
\begin{suppdash}
\item Correct: play S6\,\supparr\,S8 in order and enter saying practice.
\item Wrong on the first attempt: play S7(right) and let the child try once more.
\item Unclear pointing or no response on the first attempt: replay S4(right) and let the child try once more.
\item Still not correct on the second attempt: play S19 and end the session.
\end{suppdash}

\textbf{4. Pointing and saying.} The child chooses any word that is not finished yet, points to its card, and says the word. The system gives the corresponding feedback according to whether the actual pointing matches the independently recognized word.

When the choice or the capture is incomplete:
\begin{suppdash}
\item A word that is already finished is chosen: play S12 to lead the child to the other word; do not evaluate again.
\item The pointing is unclear: play S15 and capture again.
\item A card is chosen but the word is not heard clearly: play S17 and capture again.
\end{suppdash}

When the pointing matches the recognized word:
\begin{suppdash}
\item The current word has no earlier error: play S9 if the other word is not finished yet, otherwise play S10; record the current word as passed.
\item The current word is correct after its first error: play S11 and record the current word as passed; append S12 if the other word is not finished yet.
\end{suppdash}

When the pointing clearly does not match the recognized word:
\begin{suppdash}
\item First error on the current word: play S13 for the left card or S14 for the right card, and let the child retry.
\item Second error on the current word: play S16 to demonstrate the correction and end the practice of this word, and record it as not passed; append S12 if the other word is not finished yet.
\end{suppdash}

This step continues as long as the two words do not both have a result.

\textbf{5. End of the pair and switch to the next pair.} After both words have a result, play S6.

If there is a next pair:
\begin{suppparen}
\item Play S18.
\item Show the prepared cards of the next pair, and use the lines and the speech of that pair.
\item Confirm that the system can recognize pointing on the new cards.
\item Go back to step 1 and play only S3.
\end{suppparen}

If all word pairs are finished: play S19 and record the results of the practice.

\suppcardhead{Counting and ending rules}
\textbf{Identification stage: at most two attempts per word.}
\begin{suppdash}
\item Pointing to the wrong card, unclear pointing, and no response before the waiting time runs out each count as one unfinished identification; the different cases are counted together.
\item If any word has two unfinished identifications in a row, the whole session ends and is recorded as `identification not completed, ended early'.
\item S7 already contains the repeated question: after playing it, wait directly for the child to point, and do not play S4 again.
\end{suppdash}

\textbf{Saying stage: errors are counted for the two words separately and are not reset when the child switches words; at most two clear mismatches per word.}
\begin{suppdash}
\item Identification errors, unclear pointing, unclear speech, and technical failures do not use up the two errors allowed in saying.
\item After the second error on the current word, demonstrate the correction and end the practice of this word; do not ask for a third answer.
\item A finished pair may contain a word that was not passed; once both words have a result, the practice of the pair can end.
\end{suppdash}
\suppcardrule
\suppfirstcardpart{Success criteria}
\begin{suppenum}[midpenalty=10000]
\item Automatic adjustment of the viewing angle: Misty adjusts its position and angle by itself, so that the camera clearly sees the screen and the child's finger.
\item Correct teaching flow: the rules above for preparation, identification, saying, feedback, switching pairs, and ending are followed.
\end{suppenum}
\suppcardrule
\suppfirstcardpart{Optimization targets}
\begin{suppenum}
\item Pointing-direction accuracy: the accuracy of judging whether the user points to the left card or to the right card.
\item Spoken-word discrimination accuracy: from the user's speech, tell which of the two words of the current pair the user said. The transcript does not have to be fully correct, and the quality of the pronunciation is not judged; the point is to reduce the repeated questions caused by `cannot tell' or `told the wrong way round', so that the teaching flow can proceed normally.
\end{suppenum}
\end{supplongtaskcard}


==> sec/supp_F_ethics.tex <==
\section{Ethical Considerations}
\label{sec:supp-ethics}

All experiments evaluated robotic system performance rather than human behavior or clinical outcomes. Interactive tests were conducted by an author, who provided speech, gesture, and verification inputs solely for system evaluation. No external participants were recruited, and no human-subject study was conducted.


==> supp_preamble.tex <==

\usepackage{array}
\usepackage{tabularx}
\makeatletter
\@ifpackageloaded{verbatim}{%
  \usepackage[skins,breakable]{tcolorbox}%
}{%
  \let\supp@kept@verbatim\verbatim
  \let\supp@kept@endverbatim\endverbatim
  \expandafter\let\expandafter\supp@kept@sverbatim\csname verbatim*\endcsname
  \expandafter\let\expandafter\supp@kept@endsverbatim\csname endverbatim*\endcsname
  \let\supp@kept@@verbatim\@verbatim
  \usepackage[skins,breakable]{tcolorbox}%
  \let\verbatim\supp@kept@verbatim
  \let\endverbatim\supp@kept@endverbatim
  \expandafter\let\csname verbatim*\endcsname\supp@kept@sverbatim
  \expandafter\let\csname endverbatim*\endcsname\supp@kept@endsverbatim
  \let\@verbatim\supp@kept@@verbatim
}
\makeatother

\definecolor{suppblue}{rgb}{0.21,0.49,0.74}       %
\definecolor{suppgreen}{rgb}{0.18,0.49,0.196}
\definecolor{suppred}{rgb}{0.776,0.157,0.157}
\definecolor{suppgreenbg}{rgb}{0.934,0.959,0.936}
\definecolor{suppredbg}{rgb}{0.982,0.933,0.933}
\colorlet{suppframe}{black!40}        %
\colorlet{supptitlebg}{black!7}       %
\colorlet{supplabel}{black!60}        %
\colorlet{suppmuted}{black!60}        %
\colorlet{suppplaceholder}{black}     %

\makeatletter
\DeclareRobustCommand{\suppcode}[1]{{%
  \ifdim\f@size\p@>9.5\p@ \small\fi
  \fontencoding{T1}\fontfamily{pcr}\selectfont
  \def\_{\textunderscore\penalty\hyphenpenalty}#1}}
\makeatother
\newcommand{\suppvar}[1]{\suppcode{\{#1\}}}
\newcommand{\suppph}[1]{\textcolor{suppplaceholder}{$\langle$\textit{#1}$\rangle$}}
\newcommand{\suppmuted}[1]{\textcolor{suppmuted}{#1}}
\newcommand{\supparr}{\ensuremath{\rightarrow}}

\newcommand{\suppcardlabelfont}{\fontsize{7}{8.4}\selectfont\sffamily\bfseries}
\newcommand{\suppcardlabel}[1]{\leavevmode{\suppcardlabelfont\color{supplabel}\MakeUppercase{#1}}}

\newlist{suppenum}{enumerate}{1}
\setlist[suppenum]{beginpenalty=10000,label=\arabic*.,leftmargin=1.3em,labelwidth=0.95em,labelsep=0.35em,
  align=left,topsep=0pt,partopsep=0pt,parsep=0pt,itemsep=0pt}
\newlist{suppparen}{enumerate}{1}
\setlist[suppparen]{beginpenalty=10000,label=(\arabic*),leftmargin=1.7em,labelwidth=1.35em,labelsep=0.35em,
  align=left,topsep=0pt,partopsep=0pt,parsep=0pt,itemsep=0pt}
\newlist{suppdash}{itemize}{1}
\setlist[suppdash]{beginpenalty=10000,label=--,leftmargin=1.0em,labelwidth=0.65em,labelsep=0.35em,
  align=left,topsep=0pt,partopsep=0pt,parsep=0pt,itemsep=0pt}

\makeatletter
\newcommand{\suppcardpenalties}{\clubpenalty=\@M \@clubpenalty=\@M \widowpenalty=\@M
  \clubpenalties 3 \@M \@M 0 \widowpenalties 3 \@M \@M 0 }
\makeatother
\providecommand{\nolinenumbers}{}
\tcbset{
  suppcard/.style={
    enhanced,
    width=\linewidth,
    colback=white, colframe=suppframe, boxrule=0.5pt,
    arc=0pt, outer arc=0pt,
    left=5pt, right=5pt, top=4pt, bottom=4pt,
    lefttitle=5pt, righttitle=5pt, toptitle=2.4pt, bottomtitle=2.4pt,
    colbacktitle=supptitlebg, coltitle=black,
    fonttitle=\small\bfseries, titlerule=0.5pt,
    fontupper=\footnotesize,
    before upper={\setlength{\parindent}{0pt}\setlength{\parskip}{0pt}\raggedright\suppcardpenalties},
    before skip=6pt plus 3pt minus 1pt,
    after skip=6pt plus 3pt minus 1pt,
  }
}

\newenvironment{supptaskcard}[3][]{%
  \nolinenumbers
  \begin{tcolorbox}[suppcard,
    title={\suppcardtarget{#1}\textcolor{suppblue}{#2}\hspace{0.8em}#3}]}%
  {\end{tcolorbox}}

\newenvironment{supplongtaskcard}[3][]{%
  \nolinenumbers
  \begin{tcolorbox}[suppcard, breakable,
    title={\suppcardtarget{#1}\textcolor{suppblue}{#2}\hspace{0.8em}#3},
    title after break={\textcolor{suppblue}{#2}\hspace{0.8em}#3\hspace{0.6em}{\normalfont\footnotesize\suppmuted{(continued)}}},
    before upper={\setlength{\parindent}{0pt}\setlength{\parskip}{0.5pt plus 0.5pt}\raggedright\suppcardpenalties},
    lines before break=3]}%
  {\end{tcolorbox}}

\makeatletter
\newcommand{\suppcardtarget}[1]{\if\relax\detokenize{#1}\relax\else
  \@ifundefined{hypertarget}{}{\hypertarget{#1}{}}\fi}
\DeclareRobustCommand{\supptaskref}[2]{\@ifundefined{hyperlink}{#2}{\hyperlink{#1}{#2}}}
\makeatother

\newcommand{\suppfirstcardpart}[1]{\suppcardlabel{#1}\par\nopagebreak\vspace{1.2pt}}
\newcommand{\suppcardpart}[1]{\par\vspace{3.5pt}\suppcardlabel{#1}\par\nopagebreak\vspace{1.2pt}}
\newcommand{\suppcardpartnote}[2]{\par\vspace{3.5pt}\suppcardlabel{#1}\
  {\fontsize{7}{8.4}\selectfont\sffamily\color{supplabel}#2}\par\nopagebreak\vspace{1.2pt}}
\makeatletter
\newcommand{\suppsline}[3]{\par{\interlinepenalty=\@M \textbf{#1} #2 \suppmuted{#3}\par}}
\makeatother
\newcommand{\suppcardrule}{\par\vskip 3pt
  \cleaders\vbox to 0.4pt{\hbox to \linewidth{\color{suppframe}\leaders\hrule height 0.4pt\hfill}\vss}\vskip 0.4pt
  \vskip 3pt}
\newcommand{\suppcardhead}[1]{\par\vspace{2.5pt}\textbf{#1}\par\nopagebreak}
\newcommand{\suppcardgroup}[1]{\par\vspace{1.5pt}\textit{#1}\par\nopagebreak}

\newtcolorbox{suppverifycard}[3]{%
  enhanced, width=\linewidth,
  colback=white, colframe=black!25, boxrule=0.4pt, arc=0pt, outer arc=0pt,
  left=8pt, right=6pt, top=5pt, bottom=5pt,
  lefttitle=8pt, toptitle=3pt, bottomtitle=3pt,
  colbacktitle=#2, coltitle=black, fonttitle=\small, titlerule=0.4pt,
  fontupper=\small,
  before upper={\setlength{\parindent}{0pt}\setlength{\parskip}{2pt}\raggedright},
  borderline west={2.5pt}{0pt}{#1},
  before={\par\noindent}, after={\par},
  title={#3}}
\newcommand{\suppfirstvlabel}[1]{\suppcardlabel{#1}\par\nopagebreak}
\newcommand{\suppvlabel}[1]{\par\vspace{4pt}\suppcardlabel{#1}\par\nopagebreak}

\newcommand{\supptablesetup}{\centering\small\renewcommand{\arraystretch}{1.15}}
\newcommand{\supplisttablesetup}{\centering\footnotesize\renewcommand{\arraystretch}{1.15}}
\newcommand{\supphitem}[2]{\ifvmode\else\par\fi
  \hangindent=1.3em\hangafter=1\noindent\makebox[1.3em][l]{#1.}#2}
\newcommand{\supptablenote}[1]{\par\vspace{2pt}{\footnotesize\raggedright #1\par}}

\newcommand{\suppskillcell}[2]{\begin{tabular}[t]{@{}l@{}}\suppcode{#1}\\[-1pt]{\footnotesize\suppmuted{#2}}\end{tabular}}
\newcommand{\supptwolinehead}[2]{\begin{tabular}[b]{@{}c@{}}\textbf{#1}\\[-1.5pt]\textbf{#2}\end{tabular}}

